BGP Security in Partial Deployment: Is the Juice Worth the Squeeze?

As the rollout of secure route origin authentication with the RPKI slowly gains traction among network operators, there is a push to standardize secure path validation for BGP (i.e., S*BGP: S-BGP, soBGP, BGPSEC, etc.). Origin authentication already does much to improve routing security. Moreover, the transition to S*BGP is expected to be long and slow, with S*BGP coexisting in "partial deployment" alongside BGP for a long time. We therefore use theoretical and experimental approach to study the security benefits provided by partially-deployed S*BGP, vis-a-vis those already provided by origin authentication. Because routing policies have a profound impact on routing security, we use a survey of 100 network operators to find the policies that are likely to be most popular during partial S*BGP deployment. We find that S*BGP provides only meagre benefits over origin authentication when these popular policies are used. We also study the security benefits of other routing policies, provide prescriptive guidelines for partially-deployed S*BGP, and show how interactions between S*BGP and BGP can introduce new vulnerabilities into the routing system.

==> thebib.tex <==
\begin{thebibliography}{10}

\bibitem{IRRpt} {IRR} power tools. \newblock \url{http://sourceforge.net/projects/irrpt/}, 2011.

\bibitem{fccReport} Working group 6 secure bgp deployment report. \newblock Technical report,
    {FCC CSRIC}
  \url{http://transition.fcc.gov/bureaus/pshs/advisory/csric3/CSRICIII_9-12-12%
_WG6-Final-Report.pdf}, 2012.

\bibitem{ixpSIGCOMM12} B.~Ager, N.~Chatzis, A.~Feldmann, N.~Sarrar, S.~Uhlig, and W.~Willinger.
    \newblock Anatomy of a large european {IXP}. \newblock In {\em SIGCOMM'12}, 2012.

\bibitem{alexa} Alexa. \newblock The top 500 sites on the web. \newblock
    \url{http://www.alexa.com/topsites}, October 1 2012.

\bibitem{ixp} B.~Augustin, B.~Krishnamurthy, and W.~Willinger. \newblock {IXPs}: Mapped?
    \newblock In {\em IMC'09}, 2009.

\bibitem{JenYannis} I.~Avramopoulos, M.~Suchara, and J.~Rexford. \newblock How small groups can
    secure interdomain routing. \newblock Technical report, Princeton University Comp. Sci.,
    2007.

\bibitem{PaulF} H.~Ballani, P.~Francis, and X.~Zhang. \newblock A study of prefix hijacking and
    interception in the {I}nternet. \newblock In {\em SIGCOMM'07}, 2007.

\bibitem{robertCCS} A.~Boldyreva and R.~Lychev. \newblock Provable security of s-bgp and other
    path vector protocols: model,
  analysis and extensions.
\newblock In {\em CCS'12}, pages 541--552.

\bibitem{pakistan} M.~A. Brown. \newblock {Rensys Blog: Pakistan hijacks YouTube}. \newblock
  \url{http://www.renesys.com/blog/2008/02/pakistan_hijacks_youtube_1.shtml}.

\bibitem{BGPsurvey} K.~Butler, T.~Farley, P.~McDaniel, and J.~Rexford. \newblock A survey of
    {BGP} security issues and solutions. \newblock {\em Proceedings of the IEEE}, 2010.

\bibitem{adoptability} H.~Chang, D.~Dash, A.~Perrig, and H.~Zhang. \newblock Modeling
    adoptability of secure {BGP} protocol. \newblock In {\em SIGCOMM'06}, 2006.

\bibitem{cyclops} Y.-J. Chi, R.~Oliveira, and L.~Zhang. \newblock Cyclops: The {Internet}
    {AS}-level observatory. \newblock {\em SIGCOMM CCR}, 2008.

\bibitem{bestpath} Cisco. \newblock Bgp best path selection algorithm: How the best path
    algorithm works. \newblock Document ID: 13753, May 2012. \newblock
  \url{http://www.cisco.com/en/US/tech/tk365/technologies_tech_note09186a00800%
94431.shtml#bestpath}.

\bibitem{china} J.~Cowie. \newblock Rensys blog: China's 18-minute mystery. \newblock
  \url{http://www.renesys.com/blog/2010/11/chinas-18-minute-mystery.shtml}.

\bibitem{amogh} A.~Dhamdhere and C.~Dovrolis. \newblock Twelve years in the evolution of the
    internet ecosystem. \newblock {\em Trans. Netw.}, 19(5):1420--1433, 2011.

\bibitem{ggr} L.~Gao, T.~Griffin, and J.~Rexford. \newblock Inherently safe backup routing with
    {BGP}. \newblock {\em IEEE INFOCOM}, 2001.

\bibitem{gr} L.~Gao and J.~Rexford. \newblock Stable {Internet} routing without global
    coordination. \newblock {\em Trans. Netw.}, 2001.

\bibitem{surveyEmail} P.~Gill, S.~Goldberg, and M.~Schapira. \newblock A survey of interdomain
    routing policies. \newblock NANOG'56, October 2012.

\bibitem{adopt} P.~Gill, M.~Schapira, and S.~Goldberg. \newblock Let the market drive deployment:
    A strategy for transistioning to
  {BGP} security.
\newblock {\em SIGCOMM'11}, 2011.

\bibitem{sigBGP} S.~Goldberg, S.~Halevi, A.~D. Jaggard, V.~Ramachandran, and R.~N. Wright.
    \newblock Rationality and traffic attraction: Incentives for honest path
  announcements in {BGP}.
\newblock In {\em SIGCOMM'08}, 2008.

\bibitem{BGPattack} S.~Goldberg, M.~Schapira, P.~Hummon, and J.~Rexford. \newblock How secure are
    secure interdomain routing protocols? \newblock In {\em SIGCOMM'10}, 2010.

\bibitem{wedgies} T.~Griffin and G.~Huston. \newblock {BGP} wedgies. \newblock RFC 4264, 2005.

\bibitem{gsw} T.~Griffin, F.~B. Shepherd, and G.~Wilfong. \newblock The stable paths problem and
    interdomain routing. \newblock {\em Trans. Netw.}, 2002.

\bibitem{hustonModel1} G.~Huston. \newblock Peering and settlements - {Part I}. \newblock {\em
    The Internet Protocol Journal (Cisco)}, 2(1), March 1999.

\bibitem{hustonModel12} G.~Huston. \newblock Peering and settlements - {Part II}. \newblock {\em
    The Internet Protocol Journal (Cisco)}, 2(2), June 1999.

\bibitem{BGPSECthreat} S.~Kent and A.~Chi. \newblock Threat model for bgp path security.
    \newblock Internet draft: draft-ietf-sidr-bgpsec-threats-04, 2013.

\bibitem{SBGP} S.~Kent, C.~Lynn, and K.~Seo. \newblock Secure border gateway protocol {(S-BGP)}.
    \newblock {\em JSAC}, 2000.

\bibitem{labovitzHyperGiant} C.~Labovitz. \newblock Arbor blog: Battle of the hyper giants.
    \newblock
  \url{http://asert.arbornetworks.com/2010/04/the-battle-of-the-hyper-giants-p%
art-i-2/}.

\bibitem{labovitzPreso} C.~Labovitz. \newblock Internet traffic 2007 - 2011. \newblock Global
    Peering Forum. Santi Monica, CA., April 2011.

\bibitem{LabovitzSIGCOMM} C.~Labovitz, S.~Iekel-Johnson, D.~McPherson, J.~Oberheide, and
    F.~Jahanian. \newblock Internet inter-domain traffic. \newblock In {\em SIGCOMM'10}, 2010.

\bibitem{BGPSEC} M.~Lepinski. \newblock Bgpsec protocol specification:
    draft-ietf-sidr-bgpsec-protocol-06. \newblock Internet-Draft, 2012.

\bibitem{rpki} M.~Lepinski and S.~Kent. \newblock {\em RFC 6480: An Infrastructure to Support
    Secure Internet Routing}.

\bibitem{LGSPODC12} R.~Lychev, S.~Goldberg, and M.~Schapira. \newblock Network destabilizing
    attacks. \newblock In {\em PODC'12}, 2012.

\bibitem{full} R.~Lychev, S.~Goldberg, and M.~Schapira. \newblock Is the juice worth the squeeze?
    {BGP} security in partial deployment. \newblock Technical report, Arxiv, 2013.

\bibitem{OrAuth} P.~McDaniel, W.~Aiello, K.~Butler, and J.~Ioannidis. \newblock Origin
    authentication in interdomain routing. \newblock {\em Computer Networks}, November 2006.

\bibitem{AS7007} S.~Misel. \newblock {``Wow, AS7007!"}. \newblock Merit NANOG Archive, April
    1997. \newblock \url{http://www.merit.edu/mail.archives/nanog/1997-04/msg00340.html}.

\bibitem{pfx-validate-09} P.~Mohapatra, J.~Scudder, D.~Ward, R.~Bush, and R.~Austein. \newblock
    {\em BGP Prefix Origin Validation}. \newblock Internet Engineering Task Force Network Working
    Group, 2012. \newblock \url{http://tools.ietf.org/html/draft-ietf-sidr-pfx-validate-09}.

\bibitem{roaRPSL} P.~Palse. \newblock {Serving ROAs as RPSL route[6] Objects from the RIPE
    Database}. \newblock RIPE Labs, June 2010. \newblock
  \url{https://labs.ripe.net/Members/Paul_P_/content-serving-roas-rpsl-route-o%
bjects}.

\bibitem{moratel} T.~Paseka. \newblock Cloudflare blog: Why google went offline today., November
    2012. \newblock
  \url{http://blog.cloudflare.com/why-google-went-offline-today-and-a-bit-abou%
t}.

\bibitem{DEFCON} A.~Pilosov and T.~Kapela. \newblock Stealing the {Internet}: An {Internet}-scale
    man in the middle
  attack, 2008.
\newblock {DEFCON}'16.

\bibitem{FCCcommit} Reuters. \newblock Internet providers pledge anti-botnet effort, March 22
    2012.

\bibitem{10lessons} M.~Roughan, W.~Willinger, O.~Maennel, D.~Perouli, and R.~Bush. \newblock 10
    lessons from 10 years of measuring and modeling the internet's
  autonomous systems.
\newblock {\em JSAC}, 29(9):1810--1821, 2011.

\bibitem{sss} R.~Sami, M.~Schapira, and A.~Zohar. \newblock Searching for stability in
    interdomain routing. \newblock In {\em INFOCOM'09}, 2009.

\bibitem{sandvine} Sandvine. \newblock Fall 2012 global internet phenomena, 2012.

\bibitem{sriramBGPSECchoices} K.~Sriram. \newblock {BGPSEC} design choices and summary of
    supporting discussions. \newblock Internet-Draft: draft-sriram-bgpsec-design-choices-03,
    January 2013.

\bibitem{soBGP} R.~White. \newblock Deployment considerations for secure origin {BGP} {(soBGP)}.
    \newblock draft-white-sobgp-bgp-deployment-01.txt, June 2003, expired.

\end{thebibliography}

